Combining Model and Parameter Uncertainty in Bayesian Neural Networks

Bayesian neural networks (BNNs) have recently regained a significant amount of attention in the deep learning community due to the development of scalable approximate Bayesian inference techniques. There are several advantages of using Bayesian approach: Parameter and prediction uncertainty become easily available, facilitating rigid statistical analysis. Furthermore, prior knowledge can be incorporated. However so far there have been no scalable techniques capable of combining both model (structural) and parameter uncertainty. In this paper we introduce the concept of model uncertainty in BNNs and hence make inference in the joint space of models and parameters. Moreover, we suggest an adaptation of a scalable variational inference approach with reparametrization of marginal inclusion probabilities to incorporate the model space constraints. Finally, we show that incorporating model uncertainty via Bayesian model averaging and Bayesian model selection allows to drastically sparsify the structure of BNNs.

==> table.tex <==
\begin{table}[t]
 \caption{Alternative table: Statistical summaries  of the evaluation metrics defined in the text, across $10$ simulations, for the MNIST experiment.}
  \label{t1}
  \small
  %\centering
  %\begin{adjustbox}{angle=90}
  \begin{tabular}{lcccc}
   \toprule
   % \multicolumn{2}{c}{Part}                   \\
   % \cmidrule(r){1-2}
Metric& Med.  & Min. & Max. &ACT.W\\
    \midrule
 &   \multicolumn{4}{l}{\it Bayesian sparse NN}\\
$\text{ACC}$&0.970&0.966&0.971&0.083\\%&0.00162\\
$\text{MED-ACC}$&0.963&0.960&0.966&0.051\\%&0.00182\\ 
$\text{MEAN-ACC}$&0.971&0.967&0.970&1.000\\%&0.00198\\ 
$\text{POST-ACC}$&0.978&0.977&0.978&0.083\\%&0.00048\\
$\text{POSTMEAN-ACC}$&0.979&0.978&0.980&0.051\\%0&0.00064\\
$\rho(\gamma^{(1)}|\D)$&0.052&0.051&0.053&-\\%0.00047\\ 
$\rho(\gamma^{(2)}|\D)$&0.060&0.059&0.060&-\\%0.00028\\
$\rho(\gamma^{(3)}|\D)$&0.222&0.212&0.232&-\\%0.00635\\
\hline
 &\multicolumn{4}{l}{\it Bayesian dense NN}\\
 $\text{ACC}$&0.984&0.982&0.985&10.00\\%&-\\
$\text{MEAN-ACC}$&0.984&0.982&0.985&1.000\\%&0.00198\\
\hline
&\multicolumn{4}{l}{\it Bayesian dens NN - Gaussian mixture}\\
$\text{ACC}$&0.982&0.981&0.983&10.00\\%&-\\
$\text{MEAN-ACC}$&0.983&0.981&0.984&1.000\\%&0.00198\\
\hline
&\multicolumn{4}{l}{\it Concrete dropout}\\
$\text{ACC}$&0.984&0.896&0.986&0.820\\%-\\
$\text{MEAN-ACC}$&0.982&0.894&0.984&1.000\\%-\\
%Mean probability model accuracy&&0.17090&0.09130&0.31520&0.07514\\ 
%Median probability model accuracy&&0.09895&0.09190&0.10280&0.00353\\ 
\hline
&\multicolumn{4}{l}{\it Horseshoe prior}\\
$\text{ACC}$&0.983&0.982&0.984&1.000\\%-\\
$\text{COMPR-ACC}$&0.975&0.970&0.979&0.194\\%-\\

\bottomrule
  \end{tabular}
%\end{adjustbox}
\end{table}
